Generalizable One-shot Neural Head Avatar

We present a method that reconstructs and animates a 3D head avatar from a single-view portrait image. Existing methods either involve time-consuming optimization for a specific person with multiple images, or they struggle to synthesize intricate appearance details beyond the facial region. To address these limitations, we propose a framework that not only generalizes to unseen identities based on a single-view image without requiring person-specific optimization, but also captures characteristic details within and beyond the face area (e.g. hairstyle, accessories, etc.). At the core of our method are three branches that produce three tri-planes representing the coarse 3D geometry, detailed appearance of a source image, as well as the expression of a target image. By applying volumetric rendering to the combination of the three tri-planes followed by a super-resolution module, our method yields a high fidelity image of the desired identity, expression and pose. Once trained, our model enables efficient 3D head avatar reconstruction and animation via a single forward pass through a network. Experiments show that the proposed approach generalizes well to unseen validation datasets, surpassing SOTA baseline methods by a large margin on head avatar reconstruction and animation.

==> Preliminaries.tex <==
\section{Preliminaries}
\subsection{3D Morphable Models (3DMM)}
In this paper, we utilize the strong geometry prior from an affine-based 3DMM~\cite{deng2019accurate} that takes a portrait image as input and predicts its shape and texture by:
\begin{equation}
\begin{split}
    S &= \bar{S} + B_{id}\alpha + B_{exp}\beta \\    
    T &= \bar{T} + B_{tex}\delta
\end{split}
\end{equation}
where $\bar{S}$, $\bar{T}$ are the average shape and texture of human faces, $B_{id}, B_{exp}, B_{tex}$ are the shape, expression and texture bases, $\alpha, \beta, \delta$ are coefficients that linearly combine the shape, expression and texture bases.
%
In this paper, we mainly utilize the shape and expression knowledge provided by the 3DMM, thus we ignore the texture and illumination module in the 3DMM and simply denote the rendering operation at camera view $C$ as $I=\mathcal{R}_{M}(\alpha, \beta, C)$, where $I$ is the rendered image.

%\subsection{Tri-plane Representation and Volumetric Rendering}
%A tri-plane~\cite{Chan2022} is a compact representation of an implicit 3D volume.
%
%The key idea is to represent a 3D volume by interpolating three orthogonal 2D feature maps.
%
%In this paper, we represent 3D human head as a tri-plane for its memory efficiency and capacity in detail representation.
%


